Iso-Quality of Service: Fairly Ranking Servers for Real-Time Data Analytics

We present a mathematically rigorous Quality-of-Service (QoS) metric which relates the achievable quality of service metric (QoS) for a real-time analytics service to the server energy cost of offering the service. Using a new iso-QoS evaluation methodology, we scale server resources to meet QoS targets and directly rank the servers in terms of their energy-efficiency and by extension cost of ownership. Our metric and method are platform-independent and enable fair comparison of datacenter compute servers with significant architectural diversity, including micro-servers. We deploy our metric and methodology to compare three servers running financial option pricing workloads on real-life market data. We find that server ranking is sensitive to data inputs and desired QoS level and that although scale-out micro-servers can be up to two times more energy-efficient than conventional heavyweight servers for the same target QoS, they are still six times less energy efficient than high-performance computational accelerators.

==> enumitem/README <==
Enumitem 3.5.2
~~~~~~~~~~~~~~

A package to customize the three basic lists (enumerate,
itemize and description) by means of a set of parameters,
and to clone them to define new "logical" lists.
It provides most of the flexibility you may want to
design your own lists:
- fancy labels and fancy refs,
- leftmargin, labelsep and labelwidth automatically set,
- changes applied globally or only in one of the three
  types or even in a single list (including topsep) by
  means of a sort of "inheritance",
- inline lists,
- several description styles (which fix some bad
  spacing, too),
- starting value and counter resuming,
- trivlists properly formatted,
- control on page breaking,
- gathering of lists to be treated like a unit.

Recent changes (3.0)
~~~~~~~~~~~~~~~~~~~~

1) Inline lists, with keys to set how items are joined (ie, the
punctuation between items).  Two modes are provided: `boxed' an
`unboxed' -- with the former (the default) a different punctuation
before the last item is allowed.
2) \setlist is calc-savvy (eg, for use in loops), and you can set
diferent lists and levels at once.
3) All lengths related to labels can take the value * (and not only
labelsep and leftmargin).  Its behaviour has been made consistent and
there is new value !  which does not compute the widest label.
4) With \restartlist{list-name}, list counters can be restarted (in
case you are using `resume').
5) `resume*' can be combined with other keys.
6) Lists can be gathered globally using series, so that they are
considered a single list.  To start a series just use
series=<series-name> and then resume it with resume=<series-name> or
resume*=<series-name>.
7) The ``experimental'' fullwidth has been replaced by a new key
`wide'.
8) \SetLabelAlign defines new align values.
9) You can define ``abstract'' values (eg, label=numeric) and
new keys.

Bug fixes (3.0)
~~~~~~~~~~~~~~~

- Star values (eg, leftmargin=*) could not be overriden
and new values were ignored.
- nolistsep as the first of several keys was not always
recognized and therefore treated like a short label
(ie, nol\roman*stsep).
- labelwidth didn't always work (when there was a prior
`widest' and *)
- With align=right the label and the following text could
overlap.
- description didn't get the correct list level.
- At some point (2.x?) \value* stopped working.

3.1
~~~
- Fixed incompatibility with xkeyval

3.2
~~~
- start and widest* are calc-savvy.
- \value can be used with widest*
- Some internal restrictions in \arabic and the like has been removed.
It is more flexible at the cost of having a more ``relaxed'' error
checking.

3.3
~~~
- Using *-values with itemize and description didn't work.

3.4
~~~
- New key nosep, replacing nolistsep, which didn't work as
documented.
- Fixed spacing in inline boxed lists.
- Fixed (hopefully) the bug with noitemsep and shorlabels.

3.5.0
~~~~~
- Fixed the fix related to inline lists (spacefactor).
- Fixed some problems in nested boxed inline lists.
(- And sub-sub-versions are introduced.)

3.5.1
~~~~~
- resume* only worked once, and subsequent ones
behaved like resume.

3.5.2
~~~~~
- \setlist* didn't work.

_________________________________________________________________
Javier Bezos                    | http://www.tex-tipografia.com
.................................................................
2011-09-28





==> mc_sorted_tables.tex <==
%=======================================================================
%
%   MC TABLE(S)  
%
%=======================================================================
   %
\typeout{>>>> Processing MC tables}   
   %
\begin{table}[htbp]
   %
  \footnotesize
  \centering
  \caption{Standalone MC (N=0.5M and QoS=10\%) kernel experiments}
  \begin{tabular}{lrrrrrrr} 
     %
   \toprule
   \multicolumn{1}{l}{\bf Platform}   & 
   \multicolumn{1}{c}{\bf VEC TYPE}   & 
   \multicolumn{1}{c}{\bf S/Opt}      & 
   \multicolumn{1}{c}{\bf J/Opt}      &
   \multicolumn{1}{c}{\bf Energy(KJ)}    \\
  %
   \midrule \textbf{MC Viridis(16$\times$4$\times$1)} 
&INTRINSICS&0.0038&0.3830&239.85\\
\midrule \textbf{MC Intel(2$\times$8$\times$1)} 
&AUTOVECT&0.0044&0.3794&237.58\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$1)} 
&KNC512&0.0046&0.2234&139.92\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$2)} 
&NOVECT&0.0036&0.1856&116.26\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$4)} 
&INTRINSICS&0.0030&0.1584&99.19\\
%\midrule \textbf{MC Viridis(1x4x1)} 
%&INTRINSICS&0.0533&0.3804&0.00\\
%\midrule \textbf{MC Intel(1$\times$8$\times$1)} 
%&SSE128&0.0071&0.3120&0.00\\
%\midrule \textbf{MC Xeon Phi(1x1x1)} 
%&AUTOVECT&0.2381&5.3259&0.00\\
   %
\bottomrule
   %
\end{tabular}
   %
\label{tab:mc_0.5M_qos_10_table} 
   %
\end{table}  
   %
   %-------- Following removed 
   %
\begin{comment}
	
\begin{table}[htbp]
\footnotesize
\centering
\caption{Fastest S/Opt profiles for standalone MC (N=1M) kernel experiments}
\begin{tabular}{lrrrrrrr} 
\toprule
\multicolumn{1}{l}{\bf Platform} & 
\multicolumn{1}{c}{\bf VEC TYPE}  & 
\multicolumn{1}{c}{\bf S/Opt}  & 
\multicolumn{1}{c}{\bf J/Opt}    &
\multicolumn{1}{c}{\bf Y(QoS\%)}   &
\multicolumn{1}{c}{\bf Eopt(KJ)}    \\
%\multicolumn{1}{l}{\bf Platform}  && 
%\multicolumn{4}{c}{\bf $\bar{P}$(W)}                                           
\\ 
\midrule \textbf{MC Viridis(1x4x1)} 
&NEON128&0.1055&0.7657&0&0.00\\
\midrule \textbf{MC Intel(1$\times$8$\times$1)} 
&SSE128&0.0139&0.6232&0&0.00\\
\midrule \textbf{MC Intel(2$\times$8$\times$1)} 
&SSE128&0.0085&0.7193&0.0000&0.00\\
\midrule \textbf{MC Xeon Phi(1x1x1)} 
&INTRINSICS&0.4737&10.6637&0&0.00\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$1)} 
&NOVECT&0.0092&0.4545&0&0.00\\
\midrule \textbf{MC Viridis(16$\times$4$\times$1)} 
&INTRINSICS&0.0072&0.7398&0.0258&0.91\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$2)} 
&NOVECT&0.0067&0.3713&0.5676&13.06\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$4)} 
&NOVECT&0.0053&0.3171&69.2129&1375.19\\


\bottomrule
\end{tabular}
\label{tab:mc_1_table} 

\end{table}  
   %
\typeout{---- Starting on second MC table}
   %
   %  Second table 
   %
\begin{table}[htbp]
\footnotesize
\centering
\caption{Fastest S/Opt profiles for standalone MC (N=2M) kernel experiments}
\begin{tabular}{lrrrrrrr} 
\toprule
\multicolumn{1}{l}{\bf Platform} & 
\multicolumn{1}{c}{\bf VEC TYPE}  & 
\multicolumn{1}{c}{\bf S/Opt}  & 
\multicolumn{1}{c}{\bf J/Opt}    &
\multicolumn{1}{c}{\bf Y(QoS\%)}   &
\multicolumn{1}{c}{\bf Eopt(KJ)}    \\
%\multicolumn{1}{l}{\bf Platform}  && 
%\multicolumn{4}{c}{\bf $\bar{P}$(W)}                                           
\\ 
\midrule \textbf{MC Viridis(1x4x1)} 
&NEON128&0.2106&1.5485&0&0.00\\
\midrule \textbf{MC Viridis(16$\times$4$\times$1)} 
&INTRINSICS&0.0143&1.4654&0&0.00\\
\midrule \textbf{MC Intel(1$\times$8$\times$1)} 
&SSE128&0.0277&1.2474&0&0.00\\
\midrule \textbf{MC Intel(2$\times$8$\times$1)} 
&NOVECT&0.0164&1.4436&0&0.00\\
\midrule \textbf{MC Xeon Phi(1x1x1)} 
&KNC512&0.9478&21.3406&0&0.00\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$1)} 
&NOVECT&0.0177&0.9091&0&0.00\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$2)} 
&NOVECT&0.0129&0.7412&0&0.00\\
\midrule \textbf{MC Xeon Phi(1$\times$60$\times$4)} 
&NOVECT&0.0102&0.6398&0&0.00\\
   %
\bottomrule
\end{tabular}
\label{tab:mc_2_table} 
   %
\end{table}
   %
\end{comment}
   %
\typeout{<<<< Finished Processing MC tables}  
   %
%****************************************************************              
%
%   End of Tables
%
%****************************************************************


==> optimizations.tex <==
\section{Optimization Methodology}
\label{sec:Optimization Methodology}
Initially we developed a common C language code base implementing the 
MC and BT kernels described above to compile on 
all servers. This includes an algorithmic optimization which we 
developed for the MC kernel and which we describe below. We used the 
gcc and icc compiler suites (icc is not available
on the ARM system and gcc is not available on the Xeon Phi) to 
apply the loop unrolling and auto-vectorization facilities offered by 
each compiler to our code base. Setting command line flags on the
compiler is all that is needed to enable the automatic parallelisation.
Furthermore, we experimented with an approach in which we applied 
manual loop unrolling and direct programming with available vector 
registers and vector instructions through either assembler code or 
compiler supplied intrinsic functions which map to these assembler 
instructions. 
Our methodology is common accross all platforms although the details 
of the manual implementation differ due to the characteristics of each 
instruction set architecture. In the following sub-sections, we explain 
the salient details of how our we instantiated our optimization techniques
in each kernel. Our work reflects a fixed development effort of 
approximately forty-five days to create, optimize and test the code base. 
Better performance could perhaps be gained by investing more programmer
time to optimize code for enhanced performance. We leave this as future 
work.
\subsection{Algorithmic optimization of the Monte Carlo equation}
The $\max()$ function in the MC kernel is an 
if-statement which hampers performance and power efficiency 
optimizations, as will be clear in the results section.
Given that all variables in the MC loop are invariant except 
for the random number $x_i$, we calculated a threshold 
${\rm Thres}$ such that any $x_i$ need only be included in the 
the summation when $x_i>{\rm Thres}$. For Call options
\begin{equation}
   {\rm Thres} = 
        \frac{1}{\sigma \; \sqrt(T)} \; {\rm \log}_{\rm e}
        \frac{P}{ S {\rm e}^{ ( r - \frac{\sigma^2 T}{2} ) } }
   \label{eqn:mc_randnos_threhold}
\end{equation}
This pre-screening leads to algebraic 
simplifications facilitating loop vectorization as explained below 
and also allows several multiply operations to be factored 
outside the sum loop, which now becomes:
\begin{equation}
   \sum_{j=1}^{M} {\rm e}^{\sigma\sqrt T \; x_j}
   \label{eqn:mc_sum_exponentials}
\end{equation}
   %
where $M<N$ is the number of random numbers passing the threshold test.
The loop length is now shorter and many executions 
of the expensive ${\rm exp}()$ function are therefore avoided. We observed in 
some cases a four-fold reduction but this depends on the values of the 
input data defining equation (\ref{eqn:mc_randnos_threhold}).
\subsection{Vectorization of the Monte Carlo kernel}
We first unrolled the loop in equation \ref{eqn:mc_sum_exponentials} and then
used vectorization to expedite the work within each iteration. We compute 
the summation in single precision and on Intel SSE and
ARM NEON unrolled by a factor $4$, populating a single $128$ bit argument 
with the exponents. For the AVX implementation, we exploited the wider $256$ 
bit registers unrolling by a factor $8$.
In all cases passing the argument to the vectorized version of the Cephes 
software library~\cite{iMOS00a} allowed us to compute the exponentials in 
parallel.  
The Cephes library is an open source math library with versions tailored 
for the different vector units used in our study.
\subsection{Vectorizarion of the Binomial Tree kernel}
The dominant part the BT computation computation is an inner loop 
at each level in the latter, a step which can be expressed 
simply as 
\begin{equation}
   v_i = a v_i + b v_{i+1} \label{eqn:bt_loop}
\end{equation}
   %
Equation \ref{eqn:bt_loop} exhibits an anti-dependency between 
iterations, a feature that needs to be removed in order to boost 
performance via vectorization. Notably the GCC compiler for all 
our servers failed to recognize this vectorizing opportunity. However, 
the Intel compiler (ICC) proved to be excellent,
producing vectorized code in this case.
In our manual approach we programmed equation (\ref{eqn:bt_loop}) in 
vectorized assembly and also replicated this independently using vector 
intrinsics within the C source code.
These two handcrafted vectorization solutions overcome the apparent anti-dependency 
and enable us to compare the low-level manual assembly solution versus a more 
abstract, intrinsic-based vectorization method. 
Our handcrafted method establishes the $v_i$ and $v_{i+1}$ terms in equation 
(\ref{eqn:bt_loop}) as if they were two separate vectors held in CPU registers
so that independent multiply-add instrctions can be used to produce the result.
The following are its key steps per iteration, illustrated using Intel SSE:
\begin{itemize}
  \item partition the XMM registers into three sets and load eight double 
        precision values per iteration into one set of four XMM registers which
        we view as a unit. 
  \item avoiding repeated memory accesses, replicate the register contents into
        a separate set of four registers rearranging the contents as if performing 
        a push-up operation on the unit. One extra memory access is needed to load
        a value to fill the gap at the lower end.
  \item prepare a third set consisting of two vector registers such that 
        one holds two copies of $a$ and the other two copies of $b$. This can
        avoided in subsequent iterations.
  \item apply SSE multiply and add instructions to this register configuration 
        to compute eight values for the left hand side of equation 
        \ref{eqn:bt_loop}, where these valaues are in the first register set.
  \item store contents of the first set of registers to RAM.
\end{itemize}
On the AVX and KNC architectures, the wider registers allow for sixteen values 
to be processed in each iteration. 
Notwithstanding the availability of only single precision vector floating point 
operations on the ARM NEON unit, a number of differences in the instruction set 
architectures emerged between platforms when working at the assembler code level.
Regarding step 2, Intel SSE provides inter-lane shift operations on XMM registers 
making the task possible in three vector instructions. The AVX instruction 
set lacks inter-lane shifts on YMM registers so that an intricate sequence 
of seven permutation and blend operations are needed to perform the same operation
and this affects the results as shown later. 
In contrast, the NEON and KNC instruction sets provide a vector align/extract
operation thereby requiring just a single instruction. 
Regarding step 4, only KNC provides a \emph{fused multiply-add} operation meaning
that the step requires just two vector instructions while the others require three 
instructions.

